Sarcasm Analysis using Conversation Context

Computational models for sarcasm detection have often relied on the content of utterances in isolation. However, the speaker's sarcastic intent is not always apparent without additional context. Focusing on social media discussions, we investigate three issues: (1) does modeling conversation context help in sarcasm detection; (2) can we identify what part of conversation context triggered the sarcastic reply; and (3) given a sarcastic post that contains multiple sentences, can we identify the specific sentence that is sarcastic. To address the first issue, we investigate several types of Long Short-Term Memory (LSTM) networks that can model both the conversation context and the current turn. We show that LSTM networks with sentence-level attention on context and current turn, as well as the conditional LSTM network (Rocktaschel et al. 2016), outperform the LSTM model that reads only the current turn. As conversation context, we consider the prior turn, the succeeding turn or both. Our computational models are tested on two types of social media platforms: Twitter and discussion forums. We discuss several differences between these datasets ranging from their size to the nature of the gold-label annotations. To address the last two issues, we present a qualitative analysis of attention weights produced by the LSTM models (with attention) and discuss the results compared with human performance on the two tasks.

==> errlysis.tex <==
\subsection{Error Analysis} \label{section:ea}

We conducted an error analysis of our models, and we categorize the errors in the following categories: 

\paragraph{{\bf Missing Background Knowledge}}

Sarcasm or verbal irony depends to a large extent upon the shared knowledge of speaker and hearer (common ground) that is not explicitly part of the conversation context \citep{haverkate1990speech}. %However, it is often common for users to exploit external knowledge, such as \textit{common sense knowledge} and \textit{special knowledge} about entities or situations. W
%When a speakers articulate sarcastic utterances with such external knowledge they believe the hearers/readers are also aware of such shared knowledge.
For instance, check the following context/sarcastic reply pair from the $IAC_{v2}$ corpus.
\begin{quote}
{\bf userA:} i'm not disguising one thing. I am always clear that my argument is equal marriage for same sex couples. No one i know on my side argues simply for ``equality in marriage''. \\

{\bf userB:} Right, expect when talking about the 14th amendment, The way you guys like to define ``equal protection'' would make it so any restriction is unequal.
\end{quote}
%SM why is this message sarcastic?? You discussion below doesn't convince me it is.... 

Here, {\bf userB} is sarcastic while discussing the 14th amendment (i.e., equal protection). On social media, users often argue about different topics, including controversial ones.\footnote{As stated earlier, $IAC$ includes a large set of conversations from 4forums.com, a website for political debates \citep{justo2014extracting,walker2012corpus}.} When engaged in conversations, speakers might assume that some background knowledge about those topics is understood by the hearers (e.g., historical events). For example, posts from $Reddit$ are based on specific subreddits where users share similar interests (i.e., video games). We found, often, even if the sarcastic posts are not political, they are based on specific shared knowledge (i.e., the performance of a soccer player in recent games, sarcastic about a new video game,  etc.). LSTM or SVM models are unable to identify the sarcastic intent when such contextual knowledge that is outside of the conversation context is used by the speaker. In future, however, we intend to build a model on specific subreddits (i.e., politics, sports) to investigate how much the domain-specific knowledge helps the classifiers. 



% use this inside the model descripton Broadly speaking, \citep{wallace2015computational} have mentioned this as ``environment; something I will refer to as the pragmatic context. ''.

\paragraph{{\bf Longer Sarcastic Reply}}
Although, the $IAC_{v2}$ and $Reddit$ corpora are annotated differently (using crowdsourcing vs. self-labeled, respectively), the labels are for the posts and not for specific sentences. Thus for longer posts, often the LSTM models perform poorly since the sarcastic cue is buried under the remaining non-sarcastic parts of the post. For instance, we observe that about 75\% of the false negative cases reported by the LSTM$^{c_{a_{s}}}$+LSTM$^{r_{a_{s}}}$ on the $IAC_{v2}$ data have 5 or more sentences in the sarcastic posts. 

\paragraph{{\bf Use of Profanity and Slang}} Sarcasm could be bitter, caustic, snarky or could have a mocking intent. \citet{orabycreating} asked the annotators to look for such characteristic while annotating the $IAC_{v2}$ posts for sarcasm. We observe that although the LSTM models are particularly efficient in identifying some inherent characteristics of sarcastic messages such as ``context incongruity'' (detailed in Section \ref{section:qualitative}), they often miss the sarcastic posts that contain slang and the use of profane words. In the future, we plan to utilize a lexicon to identify such posts, similar to \citep{burfoot2009automatic}.

\paragraph{{\bf Use of Numbers}} In some instances, sarcasm is related to situations that involve numbers, and the models are unable to identify such cases (i.e., userB: ``why not? My mother has been 39, for the last 39 years.'' in reply of userA: ``actually the earth is 150 years old. fact and its age never changes''). This type of sarcasm often occurs in social media both discussion forums and Twitter  \citep{joshi2015}.   

\paragraph{{\bf Use of Rhetorical Questions}}
We also found that sarcastic utterances that use rhetorical questions ($RQ$), especially in the discussion forum (e.g., $IAC_{v2}$) are hard to identify. \citet{orabycreating} hypothesized that  sarcastic utterances of $RQ$ type are of the following structure; they contain questions in the middle of a post, that are followed by a statement. Since many discussion posts are long and might include multiple questions, question marks are not very strong indicators for $RQ$. 

%\paragraph{{\bf Use of Humor}}

%imilar to the idea of the ``narrowly-focused sarcasm''? \camp{2011}.




